Global-Order GFlowNets

Order-Preserving (OP) GFlowNets have demonstrated remarkable success in tackling complex multi-objective (MOO) black-box optimization problems using stochastic optimization techniques. Specifically, they can be trained online to efficiently sample diverse candidates near the Pareto front. A key advantage of OP GFlowNets is their ability to impose a local order on training samples based on Pareto dominance, eliminating the need for scalarization - a common requirement in other approaches like Preference-Conditional GFlowNets. However, we identify an important limitation of OP GFlowNets: imposing a local order on training samples can lead to conflicting optimization objectives. To address this issue, we introduce Global-Order GFlowNets, which transform the local order into a global one, thereby resolving these conflicts. Our experimental evaluations on various benchmarks demonstrate the efficacy and promise of our proposed method.

==> tikz/comparison.tex <==


\begin{tikzpicture}[scale=1]
  % Draw axes
  \draw[->] (0,0) -- (5,0) node[right] {$r_1$};
  \draw[->] (0,0) -- (0,4) node[above] {$r_2$};

  % Plot points with labels
  \fill (1,1) circle (2pt) node[below right] {$y_1$};
  \fill (2,1.2) circle (2pt) node[below right] {$y_2$};
  \fill (3,1.4) circle (2pt) node[below right] {$y_3$};
  \fill (4,1.6) circle (2pt) node[below right] {$y_4$};
  \fill (1.5,2) circle (2pt) node[below right] {$y_5$};
  \fill (2,3) circle (2pt) node[below right] {$y_6$};
\end{tikzpicture}


